Attacking the First-Principle: A Black-Box, Query-Free Targeted Mimicry Attack on Binary Function Classifiers

Binary function classifiers play a crucial role in maintaining the security and integrity of software systems by detecting malicious code and unauthorized modifications. However, machine learning-based classifiers are vulnerable to adversarial attacks that can evade detection. In this study, we present Kelpie, a novel framework for executing mimicry attacks, a stronger type of targeted evasion attacks, on binary function classifiers in a black-box, zero-query setting. Unlike previous approaches that rely on querying the target classifier to refine untargeted evasion attacks, Kelpie leverages code transformations that preserve the functionality of malicious payloads while causing them to be misclassified as we want. Through extensive experimentation, we demonstrate that Kelpie can successfully execute mimicry attacks against six state-of-the-art binary function classifiers representing different model architectures without requiring direct interaction with them. We further validate our approach with a practical demonstration, involving a keylogger and a wiper concealed within benign-looking functions embedded in an application. This work, to our best knowledge, is the first to demonstrate such a mimicry attack in a black-box, zero-query context, raising important questions about the reliability and security of existing machine learning-based binary function classifiers.

==> sections/background.tex <==
\subsection{Motivation}
\subsubsection*{A malicious developper's story}
s
Modern developing processes make extensive use of package managers, as they allow developers to easily reuse (hopefully) trusted, and efficient third-party code, and thus simplify their job. The package managers (ex: \textit{npm}, \textit{pip}, \textit{gem}) ecosystem have been studied~\cite{duan_deepbindiff_2020}, and several key parts where threats can arise have been analyzed. In particular, a package can be altered to contain malicious code by a contributing developer, as it was shown recently with the \textbf{xz} critical backdoor~\cite{xz}. This can be a benign package that contain a backdoor, or that will be updated to receive a "bug fix" or an "improvement" that will actually be some malicious payload. The package development server can also be compromised and allow authorized package maintainers to insert whatever code they want.\par
A malicious piece of code inserted in a larger, benign package can then be used on end users mobile app, browser or IoT device if it manages to pass through the different checks (anti-viruses, function analysis tools) along its way across the development pipeline. Do prevent this from happening, binary function analysis frameworks are being developed, leveraging the recent advances on machine learning.
\subsubsection*{SFML-classifiers}

Why select SFML-Classifiers ? Many of those models have spawned over the last decade, for a few reasons. Static analysis has its advantages on dynamic analysis: it is more secured, some code can detect that they are being executed in debug mode and not trigger the malicious behaviour. A trace may not catch the malicious behaviour, and most importantly dynamic analysis is resource intensive and heavy to setup (virtual machine to execute the binary code and monitor it). That's why many models focus on fast to obtain static features. The main weakness of static analysis is auto-modification in code, such as packers. We do not exploit this here, because we try to mimic another (benign) function and limit ourselves to the scope of a function.
There are real case scenarios of supply chain attacks triggered by a compromised binary function (\textit{payload}), injected in a benign-looking binary.
We believe that the assumption that basic features selected by SotA SFML-C can lead to correct representation of the semantics of a function program is wrong.

\subsection{Related Works}
\par Attacking machine-learning based security frameworks is a very lively topic in the community. As many research fields recently integrated machine learning to help solve related regression or classification problems, they are also making themselves vulnerable to such attacks. Some examples are speech recognition systems~\cite{schonherr_adversarial_2019}~\cite{hussain_waveguard_2021}, autonomous driving~\cite{cao_adversarial_2019}, ad blocking~\cite{tramer_adversarial_2019}, computer vision~\cite{ji_poltergeist_2021}, wireless communication systems~\cite{wang_crafting_2021}~\cite{bahramali_robust_2021}, natural language processing~\cite{boucher_bad_2021}.

\par We focus on the binary code classification task. Extracting the semantics of binary code despite its possible syntactic modifications is also a well-researched topic, and machine-learning has also been applied to try to solve this hard problem~\cite{duan_deepbindiff_2020}~\cite{marcelli_how_2022}~\cite{zuo_neural_2019}~\cite{li_palmtree_2021}. ~\cite{haq_survey_2022} Haq and Caballero conducted a binary code similarity survey in 2022, and listed 15 approaches that use machine learning.
\par Binary code analysis is key for many security applications: malware detection~\cite{dambra_decoding_2023}~\cite{zhang_enhancing_2020}, code clone detection~\cite{ding_asm2vec_2019}~\cite{xue_clone-slicer_2018}, authorship identification~\cite{alrabaee_bineye_2019}~\cite{abuhamad_large-scale_2018}~\cite{caliskan_when_2018}. Traditionally, binary code analysis is analyzed following one of two paradigms: static analysis (leveraging work on disassembly~\cite{he_debin_2018}~\cite{yu_deepdi_2022}~\cite{pang_sok_2020} and decompilation~\cite{burk_decomperson_2022}~\cite{wu_dnd_2022}) or dynamic analysis. Some work has been done to combine them~\cite{chen_symsan_2022}~\cite{vadayath_arbiter_2022}. When using machine learning, the goal is to extract interesting enough features that carry enough semantic information about the piece of code.
\par In particular, this paper focuses on \textbf{function binary code analysis}, that directly apply to important security-related problems: known library functions identifications, vulnerabilities detection~\cite{xu_patch_2020}, unknown function matching during a manual reverse-engineering process~\cite{patrick-evans_xfl_2022}, malware lineage analysis~\cite{cozzi_tangled_2020} or supply chain attacks prevention\hl{elaborate?}.

\par Here we list the different end goals of the attacks that machine learning based models have to face, the techniques used to achieve them and defend against them. Most of the time, those techniques fall in two categories: carefully crafted \textit{adversarial inputs} and \textit{poisoned models}:
% List the different objectives, and the current attacks and defenses. In each case list the different techniques used to get there.
\subsubsection*{Model inference}
Queries.
\subsubsection*{Data inference}
Queries.
\subsubsection*{Backdoor implantation}
Data poisoning.
\subsubsection*{Evasion}
Given a target trained model, the attacker want to generate an ("adversarial") example that will get misclassified. Those attacks can be gradient-based~\cite{chen_hopskipjumpattack_2020}, leverage knowledge of the target model ~\cite{wang_attacking_2019}, adapt the adversarial sample after querying the target model and observing the output~\cite{suya_hybrid_2020}~\cite{co_procedural_2019}.
Defenses include \textit{stateful defense models}~\cite{feng_stateful_2023} that look at the queries history, input feature analysis~\cite{hussain_waveguard_2021}.
\par A more advanced evasion attack is \textit{mimicry attacks}. The attacker not only tries to have its adversarial example misclassified, but also control the class to which it will be assigned~\cite{wagner_mimicry_nodate}\hl{double check that}t~\cite{goyal_sometimes_2023}, by mimicking the features of other samples.
\\
% List the different limitations
\par In those papers, the proposed threat model can be restricted with the following limitations:
\subsubsection*{Defender's model representation class}
Black-box, grey-box and white-box. We are black-box.
\subsubsection*{Queries to the defender's model}
Unlimited queries (gradient-based approaches), limited queries, no queries (no-one except us ?)
\\
% Finally, a complete description of us
\par We worked on building a framework allowing us to consistently evade selected binary code classifiers. The classifiers that we try to evade are:
\begin{itemize}
    \item Working at the \textbf{function} or \textbf{code sequence} level, not the whole binary
    \item Using \textbf{machine learning} to classify / embed such pieces of code
    \item Using \textbf{statically-extracted features} to represent such pieces of code
\end{itemize}
Moreover, as detailed in the threat model\ref{threat-model}, we are \textbf{compiler agnostic} and \textbf{don't allow ourselves to query} the defender's model.


% spearate the goals and the means of the techniques.



\par To the best of our knowledge, there are no other evasion techniques that operate in the \textbf{black-box, no query} setting and try to \textbf{mimick} selected functions. This is a novel, stronger attack.

==> sections/ethics.tex <==
% \GAB{Guideline: All submissions are required to have an ethics considerations section in the main body of the paper, or in the extra page offered for "ethics considerations and compliance with the open science policy". In some cases, the ethics discussion may be short; in other cases, the ethics consideration may be long}

\subsubsection*{Disclosure ethical consideration.}
This work falls within a long-standing line of research on classifier design and adversarial methods, a field that is particularly active not only in security but also in the broader machine learning community.

The primary objective of this study is to identify and understand the fundamental flaw in machine learning-based defense systems that could be exploited by malicious actors. By proactively uncovering these weaknesses, researchers and practitioners can develop more effective defenses and enhance model robustness.

At the same time, we are aware that the development of evasion attacks could potentially aid malicious actors.

However, such dual-use scenarios are common in the field of security, and the community generally agrees that open research provides more benefits than harm.



% 
%While developing evasion attacks on machine learning classifiers may appear to be potentially dangerous, here in the context of supply chain attacks, such research is crucial for enhancing the security and robustness of AI systems, that are nowadays ubiquitous.

%Moreover, sharing findings from such studies with the broader academic and professional communities can raise an alarm about existing security gaps, leading to stronger defenses against real-world attacks.

%\subsubsection*{Other ethical concerns.}
%We do not believe to have crossed other ethical concerns with our current work.

\subsubsection*{Compliance with open science policy.} We will adhere to the following measures to promote open science and the reproducibility of scientific work.

% \GAB{Research results should be available to the public or explain why this is not possible. The artifact evaluation process is adjusted to accommodate this.}

\noindent
{\em Availability.} The prototype implementation of \kelpiewill be released as an open-source framework. We will also release all the datasets, classifiers, and scripts used in this paper for scientific evaluation.

\noindent
{\em Reproducibility.} 
Reproducing our benchmark entirely from scratch may be challenging due to several components in the pipeline that require the use of licensed software, such as IDAPro for disassembly. We will provide intermediate files containing processed data that are not subject to licensing restrictions, allowing researchers to reproduce our results without the need for third-party software dependencies.
